Toward Depth Estimation Using Mask-Based Lensless Cameras

Recently, coded masks have been used to demonstrate a thin form-factor lensless camera, FlatCam, in which a mask is placed immediately on top of a bare image sensor. In this paper, we present an imaging model and algorithm to jointly estimate depth and intensity information in the scene from a single or multiple FlatCams. We use a light field representation to model the mapping of 3D scene onto the sensor in which light rays from different depths yield different modulation patterns. We present a greedy depth pursuit algorithm to search the 3D volume and estimate the depth and intensity of each pixel within the camera field-of-view. We present simulation results to analyze the performance of our proposed model and algorithm with different FlatCam settings.

==> depth.tex <==

The model in \eqref{eq:planarMeasuerments} assumes a 2D scene that consists of a single plane at some fixed depth. The system matrix $\Phi$ encodes mapping of scene points from that plane to the sensor pixels. In our new model, we consider a 3D scene that consists of multiple planes, each of which contribute to the sensor measurements. Without loss of generality, we consider a 1D imaging system in Fig.~\ref{fig:3Dgeometry} and assume that the sensor plane is centered at the origin and the mask plane is placed in front of it at distance $d$. The scene consists of $K$ planes at depths $[D_1,\ldots,D_K]$ and the scene pixels are distributed uniformly along angles in interval $[\theta_-,\theta_+]$, as before. We can describe the measurement at sensor pixel $s$ as
\begin{equation}\label{eq:depthMeasurements}
y(s) = \sum_{D = D_1}^{D_K} \sum_{\theta = \theta_-}^{\theta_+} \varphi(s,\theta,D) x(\theta,D),
\end{equation}
where $\varphi(s,\theta,D)$ denotes modulation coefficient of the mask for a light ray between scene pixel at $x(\theta,D)$ and the sensor pixel at location $s$. We can write 
\eqref{eq:depthMeasurements} in a compact form as 
\begin{equation}
y = \sum_{D=D_1}^{D_M} \Phi_D x_D,
\end{equation}
where each $x_D$ denotes intensity of $N$ pixels in a plane at depth $D$ and $\Phi_D$ is an $M\times N$ matrix that represents the mapping of $x_D$ onto the sensor. 

Furthermore, we can include multiple cameras at different locations and orientations with respect to a reference frame. Such a system will provide us multiple sensor measurements of the form 
\begin{equation}\label{eq:depthMultipleCam}
y_c = \sum_{D=D_1}^{D_M} \Phi_{D,c} x_D,
\end{equation}
where $y_c$ denotes sensor measurements at camera $c$ and $\Phi_{D,c}$ is matrix that represents mapping of $x_D$ onto camera $c$. 


\paragraph{Joint image and depth reconstruction} We estimate the depth and intensity of each pixel within the field-of-view of our cameras using a \textit{greedy depth-selective algorithm}. We estimate $x$ from \eqref{eq:depthMultipleCam} for all $(\theta,D)$ by assuming a sparse prior such that $x(\theta,D)$ is nonzero only for one depth. We also consider occlusion of the points and give a higher preference for planes closer to the sensor. A simulation result of our algorithm is given in Fig.~\ref{fig:results}. 



\paragraph{Depth sensitivity}
For a single camera, sensor measurements for a single point source at location $(\theta,D)$ can be described as 
\begin{equation}
y(s) = \text{mask}\left[\left(1-\frac{d}{D}\right) s + d\sin \theta\right].
\end{equation}
We use this relation to divide the scene into planes at non-uniform depths and uniform angles to model the 3D space within camera field-of-view. 
% The points at the same depth and different angles cast shadows that are shifted versions of one another. Points along the same angle with respect to the center of the sensor cause the same shift in the mask shadow. 



\begin{figure*}
	\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\includegraphics[width=\linewidth]{testImage}
		\caption{Test image with three cards placed at three different depths.}
		\label{fig:testImage}
	\end{subfigure}
	\hspace{5pt}
	%
	\begin{subfigure}[t]{0.3\textwidth}
		\includegraphics[width=\linewidth]{recDepthScanImage}
		\caption{Image reconstructed by assuming that the scene consists of a single plane at a fixed depth.}
		\label{fig:testImage}
	\end{subfigure}
	\hspace{5pt}
	%
	\begin{subfigure}[t]{0.3\textwidth}
		\includegraphics[width=\linewidth]{recDepthSelectImage}
		\caption{Image reconstructed using depth-selective algorithm that jointly estimates the depth and intensity of each pixel.}
		\label{fig:testImage}
	\end{subfigure}
	\caption{Simulation results to demonstrate the effect of depth sensitivity and a result for our joint depth and intensity reconstruction algorithm.}	\label{fig:results}
	\vspace{-10pt}
\end{figure*}

